DreamLLM: Synergistic Multimodal Comprehension and Creation

This paper presents DreamLLM, a learning framework that first achieves versatile Multimodal Large Language Models (MLLMs) empowered with frequently overlooked synergy between multimodal comprehension and creation. DreamLLM operates on two fundamental principles. The first focuses on the generative modeling of both language and image posteriors by direct sampling in the raw multimodal space. This approach circumvents the limitations and information loss inherent to external feature extractors like CLIP, and a more thorough multimodal understanding is obtained. Second, DreamLLM fosters the generation of raw, interleaved documents, modeling both text and image contents, along with unstructured layouts. This allows DreamLLM to learn all conditional, marginal, and joint multimodal distributions effectively. As a result, DreamLLM is the first MLLM capable of generating free-form interleaved content. Comprehensive experiments highlight DreamLLM's superior performance as a zero-shot multimodal generalist, reaping from the enhanced learning synergy. Project page: https://dreamllm.github.io.

==> useful_package.tex <==
% Useful packages and definitions during writing
% Author: Runpei Dong

% for personalized footnotes of authors info
 \makeatletter
\def\@fnsymbol#1{\ensuremath{\ifcase#1\or \star\or \dagger\or
  \mathsection\or \mathparagraph\or \|\or **\or \dagger\dagger
  \or \ddagger\ddagger \else\@ctrerr\fi}}
\makeatother

% for wrapfig tables
\makeatletter
\def\@captype{table}
\makeatother

% \renewcommand{\rmdefault}{ptm}
% \renewcommand{\sfdefault}{phv}
\usepackage{ascii}
\usepackage{subfig}
\usepackage[utf8]{inputenc} % allow utf-8 input
\usepackage[T1]{fontenc}    % use 8-bit T1 fonts
% \renewcommand\ttdefault{cmtt} % set typewriter font
\usepackage{url}            % simple URL typesetting
\usepackage{booktabs}       % professional-quality tables
\usepackage{amsfonts}       % blackboard math symbols
\usepackage{nicefrac}       % compact symbols for 1/2, etc.
\usepackage{microtype}      % microtypography
% \usepackage{bbding}         % !! this cannot be used with some packages
\usepackage{float}
\usepackage{enumerate}
\usepackage{ntheorem}
\usepackage{makecell}
\usepackage{marvosym} % \Letter
\usepackage{xfrac}
\usepackage{physics} % \grad
\usepackage{tabularx}
\usepackage{tikz}
\usepackage{bbm}
\usepackage{bm}

\newtheorem{theorem}{Theorem}
\newtheorem{definition}{Definition}
\newtheorem{lemma}{Lemma}
\newtheorem{proposition}{Proposition}
\newtheorem*{proofnn}{Proof}
\newcommand{\coo}{\ensuremath{\mathrm{CO_2}}}

\usepackage{arydshln}
\usepackage{colortbl}
\usepackage{enumitem}
\usepackage{wrapfig}
\usepackage{amsmath}
\usepackage{amssymb}
\usepackage{pifont}
\usepackage{wasysym}
\usepackage{mathrsfs}
\usepackage{multirow}
\usepackage{multicol}
\usepackage{textcomp}
\usepackage{footnote}
\usepackage{epigraph}
\usepackage{soul}
\usepackage{color}
\usepackage{xspace}
\usepackage{array}
\usepackage{threeparttable}
\usepackage[ruled,vlined]{algorithm2e} 
\newcolumntype{C}[1]{>{\centering\arraybackslash}p{#1}}
% \usepackage[pdftex]{graphicx} 

% colors
\definecolor{mydarkblue}{rgb}{0,0.08,0.55}
\definecolor{drp-blue}{HTML}{1f77b4}
\definecolor{mygray}{gray}{.9}
\definecolor{light-gray}{gray}{0.5}
\definecolor{pretty-blue}{RGB}{0, 113, 188}
\definecolor{linecolor1}{gray}{.95} % soft gray
\definecolor{linecolor}{gray}{.895} % soft gray
\definecolor{kaiming-green}{RGB}{57,181,74} % kaiming green
\definecolor{icmlblue}{rgb}{0,0.08,0.45} % ICML Blue
\definecolor{prompt_blue}{HTML}{1f78b4}
\definecolor{prompt_red}{HTML}{d45c43}
\def\eg{{\it{e.g.}}}
\def\etal{{\it{et al.}}}
\def\ie{{\it{i.e.}}}
\def\etc{{\it{etc}}}
\newcommand{\valstd}[2]{$#1 {\scriptstyle \,\pm\, #2}$}
\newcommand{\valstdb}[2]{$\mbf{#1} {\scriptstyle \,\pm\, #2}$}

\newcommand{\tablestyle}[2]{\setlength{\tabcolsep}{#1}\renewcommand{\arraystretch}{#2}\centering\footnotesize}

% \newcommand{\cmark}{\ding{51}\xspace}%
% \newcommand{\cmarkg}{\textcolor{lightgray}{\ding{51}}\xspace}%
% \newcommand{\xmark}{\ding{55}\xspace}%
% \newcommand{\xmarkg}{\textcolor{lightgray}{\ding{55}}\xspace}%

\usepackage{pifont}% http://ctan.org/pkg/pifont
\newcommand{\cmark}{{\ding{51}}}%
\newcommand{\xmark}{{\ding{55}}}%

% this is mainly for a different texttt font
\usepackage{listings}
\usepackage{lstautogobble}  %
\usepackage{color}          %
\usepackage{zi4}            %
\definecolor{bluekeywords}{rgb}{0.13, 0.13, 1}
\definecolor{greencomments}{rgb}{0, 0.5, 0}
\definecolor{redstrings}{rgb}{0.9, 0, 0}
\definecolor{graynumbers}{rgb}{0.5, 0.5, 0.5}
\definecolor{runpei-orange}{RGB}{238,133,62} % runpei orange
\lstset{
    autogobble,
    columns=fullflexible,
    showspaces=false,
    showtabs=false,
    breaklines=true,
    showstringspaces=false,
    breakatwhitespace=true,
    escapeinside={(*@}{@*)},
    commentstyle=\color{greencomments},
    keywordstyle=\color{bluekeywords},
    stringstyle=\color{redstrings},
    numberstyle=\color{graynumbers},
    basicstyle=\ttfamily\footnotesize,
    frame=l,
    framesep=12pt,
    xleftmargin=12pt,
    tabsize=4,
    captionpos=b
}

% some math def
\newcommand{\x}[0]{\mathbf{x}}
\newcommand{\w}[0]{\mathbf{w}}
\newcommand{\z}[0]{\mathbf{z}}
\newcommand{\xt}[0]{{\x}_t}
\newcommand{\wt}[0]{{\w}_t}
\newcommand{\xz}[0]{{\x}_0}
\newcommand{\xT}[0]{{\x}_T}
\newcommand{\wT}[0]{{\w}_T}
\newcommand{\zt}[0]{{\z}_t}
\newcommand{\zT}[0]{{\z}_T}
\newcommand{\zs}[0]{{\z}_{t-1}}
\newcommand{\zp}[0]{{\z}_{t+1}}
\newcommand{\bmepslion}[0]{\bm{\epsilon}}
